A Lay User Explainable Food Recommendation System Based on Hybrid Feature Importance Extraction and Large Language Models

Large Language Models (LLM) have experienced strong development in recent years, with varied applications. This paper uses LLMs to develop a post-hoc process that provides more elaborated explanations of the results of food recommendation systems. By combining LLM with a hybrid extraction of key variables using SHAP, we obtain dynamic, convincing and more comprehensive explanations to lay user, compared to those in the literature. This approach enhances user trust and transparency by making complex recommendation outcomes easier to understand for a lay user.

==> sections/OLD_relatedwork.tex <==
\section{Related Work}\label{sec:related-work}

REYHAN: I copied the content of the related work in our PRIMA paper. This section should be extended. Melisa, what is the new content that you were planning to add ?


\input{sections/primarelated}
\section{State of the art} 

\subsection{User-Centered Explanations}
This approach aims to pragmatically address a question, considering pragmatism to be synonymous with user-centeredness. It can be achieved within an explanatory process through an adequate amount of usability. In short, the definition of usability adopted in the literature is the combination of effectiveness, efficiency, and satisfaction, as per ISO 9241-210, which defines usability as "the extent to which a system, product, or service can be used by specified users to achieve specified goals with effectiveness, efficiency, and satisfaction in a specified context of use." What is crucial for proper user-centeredness is to assist the user in achieving their own goals. In an explanatory process, a user's goals are identified through questions. Some questions may be explicit, while others may not be, and their importance may diminish or increase over time. However, users are generally fully satisfied with explanations only when they effectively provide comprehensive coverage of relevant answers for all their goals \citep{sovrano2022generating}.

\subsection{Approximation with one tree} 
Decision Tree (DT) or Single Tree. It is commonly recognized that decision tree is one of the more interpretable and easily understandable models, primarily for global, but also for local, explanations. Indeed, a very widespread technique for opening the black box is the so-called “single-tree approximation” \citep{guidotti2018survey}.

\subsection{Contrastive Explanations}
Human explanations tend to be contrastive, comparing a certain factual phenomenon with a hypothetical one. In the case of decision support systems (DSS), a natural question to ask is "Why this recommendation?" This question implies a contrast, as the person asking it often has an explicit alternative in mind. In other words, the implicit question is "Why this recommendation and not that other recommendation?" The specific contrast allows the explanation to focus on the differences between the fact and the hypothesis. Humans use contrastive explanations to concisely and specifically explain events, and this advantage also applies to systems: contrastive explanations reduce the available information to a concrete difference between two outcomes. The specifics can vary depending on how the recommendation is contrasted with a different recommendation, for example, using rules or examples. In the context of a DSS recommending an insulin dose for managing type 1 diabetes, a contrastive explanation based on rules could be: "Currently, the temperature is below 10 degrees, and a lower insulin dose is recommended. If the temperature were above 30 degrees, a normal insulin dose would have been recommended." This explanation contains two rules that explicitly describe the differentiating decision boundaries between the fact and the hypothesis \citep{van2021evaluating}. In summary, facts supporting one decision are sought and counter-arguments opposing the other decision are identified \citep{padhiar2021semantic}.

\subsection{Content-Based Explanations}
Content-based explanations in recommendation systems rely on item properties and user ratings to justify recommendations. These systems use user ratings to create a classifier that represents the user's rating behavior. This classifier is then used to predict the highest ratings for recommended items \citep{tintarev2015explaining}. For example, some approaches infer a user's preferred actor based on their ratings and justify a movie recommendation based on the presence of that actor.



\subsection{Knowledge-Based Explanations}
Knowledge-based systems utilize a knowledge base and rules in an inference engine to solve problems. For example, in a knowledge-based recommendation system for cameras, properties such as memory, resolution, and price may be taken into account along with user preferences. The system can explain a camera recommendation by stating, "Less memory, lower resolution, and cheaper" \citep{tintarev2015explaining}.

\subsection{Example-Based Explanations}
Example-based explanations refer to historical situations in which the recommendation has been either true or false. For instance, "The temperature is currently 8 degrees, and a lower insulin dose is recommended. Yesterday was similar: it was 7 degrees, and the same advice turned out to be correct. Two months ago, when it was 31 degrees, a normal dose was recommended instead, which proved to be correct for that situation." Such example-based or instance-based explanations are often used among humans as they illustrate past behaviors and allow generalization to new situations \citep{van2021evaluating}.

\subsection{Contextual Explanations}
A contextual explanation provides the user with all the "external factors" that influence the decision. For example, in the given example, the season during which cauliflower is available would be considered a contextual knowledge that can be used to provide a contextual explanation, explaining why it is recommended to have potato-curry with cauliflower \citep{padhiar2021semantic}.



\subsection{Counterfactual Explanations}
Counterfactual explanations address "What if?" questions, seeking to answer whether a change would occur if the system used question parameters for a recommendation. They provide an approximation of the effects of modifying the inputs to the system. In this case, to provide an explanation, we would need to explore the effects of changing factors in the user and system profile. This can include the user's nutritional goals, preferences and dislikes, as well as any restrictive conditions such as pregnancy, allergies, and dietary requirements. For example, if a recommendation system suggests a specific dish, a counterfactual explanation could explore what would have happened if the user's preferences or constraints were different, such as in the case of pregnancy or food allergies \citep{padhiar2021semantic}.

It should be noted that contrastive explanations focus on comparing real options, whereas counterfactual explanations focus on the hypothetical consequences of changing the inputs to the system.

Most existing research has focused on exploring how users prefer a system to reason. For example, users prefer an example-based spam filter over rule-based ones \citep{pazzani2000representation}, while they prefer rule-based explanations for spam filters \citep{stumpf2009interacting}." 

\section{Evaluation of XAI Methods}

Many measures exist for computational experiments on suggested XAI methods (e.g., fidelity, sensitivity, and consistency). However, there is a lack of validated measures for user evaluations. In the literature, two main types of measures useful for user evaluations of XAI have been identified: declarative measures and behavioral measures.

\subsection{Declarative Measures}
Declarative measures are subjective and are often used in user evaluations of XAI. They provide insights into users' conscious thoughts, opinions, and perceptions. They recommend the use of declarative measures for subjective constructs (e.g., perceived understanding) but also suggest a critical perspective on whether the measures effectively address the intended constructs \citep{van2021evaluating}.

Suppose we are developing an XAI system that provides explanations for predictions made by an AI model in the medical domain. To evaluate our perception as users regarding the quality of the provided explanations, we can conduct a study where we are asked to fill out a questionnaire after interacting with the XAI system.

\subsection{Behavioral Measures}
Behavioral measures have a more observational nature and are used to measure actual behavioral effects. They recommend their use for objectively measuring constructs such as understanding and task performance. However, it is important to note that such measures often only capture one aspect of behavior \citep{van2021evaluating}.

Suppose we are developing an XAI system that generates explanations for decisions made by an AI model. To evaluate the effectiveness of this XAI system, we could conduct an experiment where we divide participants into two groups: one group uses the XAI system to obtain explanations for the model's decisions, while the other group does not have access to these explanations. We can then measure the participants' behavior, such as observing how often they request additional explanations, how many decisions they question, or how much time they spend interacting with the XAI system. These behavioral measures allow us to directly observe the effects of the XAI system on users' actual behavior when interacting with the provided explanations. They provide an objective evaluation of the impact of the XAI system on user behavior and complement the declarative measures that rely on users' subjective opinions and perceptions.

Ideally, a combination of both types of measures should be used to evaluate effects on both user perception and behavior. This way, a comprehensive perspective on a construct can be obtained. In practice, some constructs lend themselves more to declarative measures, such as user perception of confidence or understanding. Other constructs are better suited for behavioral measures, such as task performance, simulability, predictability, and persuasiveness.

Furthermore, it is recommended to measure the effects of explanations implicitly rather than explicitly. When participants are unaware of the evaluation's purpose, their responses may be more authentic. Additionally, when measuring understanding or similar constructs, explicit participant focus on the explanations can lead to biased results that do not reflect real-world application \citep{van2021evaluating}.


\newpage
\section{linked related work} 

Previous research has demonstrated that users have a growing interest in obtaining both answers and the underlying reasoning for their nutrition and food-related inquiries \citep{forbes2011content}, \citep{ueda2014recipe}, \citep{mokdara2018personalized}, \citep{ueda2011user}, \citep{el2012food}, \citep{teng2012recipe}. However, users now desire a deeper understanding of the evidence and reasoning behind these claims. In the field of food and culinary arts, efforts have been made to apply logic, reasoning, and querying techniques to capture and integrate information from diverse food-related sources \citep{haussmann2019foodkg}, \citep{haussmann2019foodkg}, \citep{batra2020recipedb}, \citep{popovski2019foodontomap}.

Existing approaches to food recommendations often rely on factors such as recipe content (e.g., ingredients) \citep{forbes2011content},\citep{el2012food}, \citep{teng2012recipe}, user behavior history (e.g., eating history) \citep{ueda2014recipe}, \citep{mokdara2018personalized}, or dietary preferences \citep{mokdara2018personalized}, \citep{ueda2011user}. However, these systems typically lack the provision of explanations for why specific food items are recommended. This limitation arises due to the utilization of black-box deep learning models, which do not offer insights into the underlying rationale behind the recommendations.

Conversely, in other domains, there are systems that employ post hoc explainable artificial intelligence (XAI) methods to provide explanations for opaque AI systems \citep{adadi2018peeking}, \citep{dovsilovic2018explainable}. However, such methods have not yet been extensively applied in the domain of food recommendation. The absence of XAI-based explanations in this domain highlights an opportunity to enhance the transparency and understanding of food recommendation systems \citep{adadi2018peeking}, \citep{dovsilovic2018explainable}. 

We were inspired by the system proposed by \citep{dragoni2020explainable}.It relies on templates, which serve as a grammar that encompasses the various elements of a persuasion message. These templates have terminal symbols organized in a hierarchical manner, with the most specific terms linked to particular persuasion strategies. A filler layer is responsible for populating the terminal symbols within the templates. Once the templates are filled, a sentence realizer generates natural language sentences that adhere to the grammatical rules of the target language. 
Our approach distinguishes itself from previous works by incorporating a higher level of explicit interpretability to food recommendations by displaying hybrid explanaition styles. This enriched approach serves as the basis for generating detailed explanations when recommending a specific food item or addressing specific questions related to a recommendation. In addition, there is a growing recognition of the importance of providing user-centered explanations that foster trust and enhance understanding of AI systems and the information they utilize for making recommendations \citep{mittelstadt2019explaining}.It also aim to address questions pragmatically, with a focus on user needs and goals \citep{sovrano2022generating}.These explanations prioritize assisting users in achieving their goals, ensuring comprehensive coverage of relevant answers for all user goals. In the pursuit of user-centered explanations, the single-tree approximation or decision trees (DT) are commonly used as interpretable models. Decision trees provide both global and local explanations and are recognized for their ease of understanding. The "single-tree approximation" technique is often employed to enhance interpretability \citep{guidotti2018survey}.Human explanations tend to be contrastive, comparing a certain factual phenomenon with a hypothetical one focusing on the differences between recommendations and alternatives. Contrastive explanations can utilize rules or examples to highlight differentiating decision boundaries \citep{van2021evaluating}. In summary, facts supporting one decision are sought and counter-arguments opposing the other decision are identified \citep{padhiar2021semantic}. 


New references/ Explain the two styles and the difference between them **********
\section{Contrasive / counterfactual explanations}
In recent years, there has been an increasing focus in the fields of philosophy of science on theories of contrastive explanations and counterfactual causality \citep{kment2006counterfactuals,ruben2015explaining}. These theories argue that causal explanations inherently involve the consideration of counterfactual cases, involving causes or events that did not actually occur. An example often cited is Lipton's (1990) \citep{lipton1990contrastive}idea that explaining why P rather than Q requires pointing out a causal difference between P and not-Q, involving a cause of P and the absence of a corresponding event in the history of not-Q. Some authors go as far as claiming that all questions about causality are fundamentally contrastive \citep{lewis1973counterfactuals,ruben2015explaining}.

However, contrastive theories of explanation have not been without criticism. \citep{ruben2015explaining} suggests that even if causal explanations are inherently contrastive (which he doubts), traditional theories of explanation can handle this aspect, making the "contrastive turn" interesting but ultimately unnecessary. While the usefulness of contrastive theories is still a topic of debate, the fact that contrastive explanations focus on specific events or cases and are thus simpler to generate than complete or global explanations of model functionality suggests that they should be further considered in the context of explainable artificial intelligence (xAI) \citep{lipton1990contrastive}.

A recent review by \citep{miller2019explanation} provides empirical evidence supporting the practical utility of everyday contrastive explanations. Miller's review encompassed articles and empirical studies from philosophy, psychology, and cognitive science that explored how individuals define, select, evaluate, and present explanations. Three primary characteristics of explanations emerged from his analysis, highlighting their real-world usage: Human explanations are contrastive, human explanations are selective, human explanations are social.




==> sections/algorithms.tex <==

% Language setting
% Replace `english' with e.g. `spanish' to change the document language

% Set page size and margins
% Replace `letterpaper' with `a4paper' for UK/EU standard size
% \usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% Useful packages
% \usepackage{amsmath}
% \usepackage{graphicx}
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\
% \usepackage[colorlinks=true, allcolors=blue]{hyperref}

\newcommand*{\argminl}{\argmin\limits}
\newcommand*{\argmaxl}{\argmax\limits}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

%\title{Your Paper}
%\author{You}

% \begin{document}



\subsection{Algorithms}

%% ITEM BASED / USER BASED EXPLANATIONS


\\
%%\begin{algorithm}
%%\label{item-based-explanations}
%%    \caption{Item-based Tags Importance extraction}
%%    \begin{algorithmic}[1]
%%        \KwData{Recipes with tags (10 recommanded and 10 not recommanded), recipeid}
%%        \KwResult{Feature importance }
%%        
%%        \STATE Delete irrelevent attributes
%%        
%%        \STATE // Train the decision tree classifier \newline
%%        \STATE clf $\leftarrow$ decisiontreeClassifier() ;
%%        \STATE clf.fit(Recipes, tags)
%%        
%%        \STATE // Get the importance of features for the recipe with "recipeid"
%%        \STATE featureImportance $\leftarrow$ clf.featuresimportance()
%%        
%%        \STATE // Print the feature in their importance order        
%%    \end{algorithmic}
%%\end{algorithm}
%%\\
%%\\
%%\\
%%\begin{algorithm}
%%\label{user-based-explanations}
%%    \caption{User-based Tags Importance extraction}
%%    \begin{algorithmic}[1]
%%        \KwData{Users informations with tags (the accepted recommanded recipe), userid}
%%        \KwResult{Feature importance }
%%        
%%        \STATE Delete irrelevent attributes
%%        
%%        \STATE // Train the decision tree classifier \newline
%%        \STATE clf $\leftarrow$ decisiontreeClassifier() ;
%%        \STATE clf.fit(Recipes, tags)
%%        
%%        \STATE // Get the importance of features for the user with "userid"
%%        \STATE featureImportance $\leftarrow$ clf.featuresimportance()
%%        
%%        \STATE // Print the feature in their importance order 
       
%%    \end{algorithmic}
%%\end{algorithm}
%%\\
%%\\
%%\\
%\begin{algorithm}[H]
%\label{counter-example-grammar-algorithm}
%    \SetAlgoLined
%    \KwData{Attributs: attr1, attr2, attr3, attr4}
%    \KwResult{Counterfactual Explanation Grammar}
%    
%    \SetKwData{avgRate}{avgRate}
%    \SetKwData{prepTime}{prepTime}
%    \SetKwData{cookTime}{cookTime}
%    \SetKwData{ovenTemp}{ovenTemp}
%    \SetKwData{sugar}{sugar}
%    \SetKwData{cholesterol}{cholesterol}
%    \SetKwData{protein}{protein}
%    \SetKwData{calories}{calories}
%    \SetKwData{recommendations}{recommendations}
%    \SetKwData{reasons}{reasons}
%    \SetKwData{taste}{taste}
%    \SetKwData{but}{but}
%    \SetKwData{recipe}{recipe}
%    \SetKwData{dislike}{dislike}
%    \SetKwData{contains}{contains}
%    \SetKwFunction{concatenateSentences}{ConcatenateSentences}
%    
%    \BlankLine
%    
%    \tcp{Initialization of rephrasing lists}
%    Initialize lists with 30 sentences for \avgRate, \prepTime, \cookTime, \ovenTemp, \sugar, \cholesterol, \protein, \calories, \recommendations, \reasons, \taste, \but, \recipe, \dislike, \contains\;
%    
%    \BlankLine
%    
%    \tcp{Random selection of a phrase from each list}
%    $randomAvgRate \leftarrow$ randomly select a sentence from \avgRate\;
%    $randomPrepTime \leftarrow$ randomly select a sentence from \prepTime\;
%    $randomCookTime \leftarrow$ randomly select a sentence from \cookTime\;
%    $randomOvenTemp \leftarrow$ randomly select a sentence from \ovenTemp\;
%    $randomSugar \leftarrow$ randomly select a sentence from \sugar\;
%    $randomCholesterol \leftarrow$ randomly select a sentence from \cholesterol\;
%    $randomProtein \leftarrow$ randomly select a sentence from \protein\;
%    $randomCalories \leftarrow$ randomly select a sentence from \calories\;
%    $randomRecommendation \leftarrow$ randomly select a sentence from \recommendations\;
%    $randomReason \leftarrow$ randomly select a sentence from \reasons\;
%    $randomTaste \leftarrow$ randomly select a sentence from \taste\;
%    $randomBut \leftarrow$ randomly select a sentence from \but\;
%    $randomRecipe \leftarrow$ randomly select a sentence from \recipe\;
%    $randomDislike \leftarrow$ randomly select a sentence from \dislike\;
%    $randomContains \leftarrow$ randomly select a sentence from \contains\;
%    
%    \BlankLine
%    
%    \tcp{Concatenation of selected sentences}
%    \Return{$randomRecommendation +  randomRecipe + randomReason + randomTaste + randomAvgRate + randomPrepTime + randomCookTime + randomOvenTemp + randomSugar + randomCholesterol + randomProtein + randomCalories + randomBut + randomContains + attr4$}
%    
%    \caption{Counterfactual Explanations Grammar Structure}
%\end{algorithm}
%\end{document} 

==> sections/backup.tex <==
\section{Related Work}\label{sec2}

REYHAN: I copied the content of the related work in our PRIMA paper. This section should be extended. Melisa, what is the new content that you were planning to add ?


\input{sections/primarelated}
\section{State of the art} 

\subsection{User-Centered Explanations}
This approach aims to pragmatically address a question, considering pragmatism to be synonymous with user-centeredness. It can be achieved within an explanatory process through an adequate amount of usability. In short, the definition of usability adopted in the literature is the combination of effectiveness, efficiency, and satisfaction, as per ISO 9241-210, which defines usability as "the extent to which a system, product, or service can be used by specified users to achieve specified goals with effectiveness, efficiency, and satisfaction in a specified context of use." What is crucial for proper user-centeredness is to assist the user in achieving their own goals. In an explanatory process, a user's goals are identified through questions. Some questions may be explicit, while others may not be, and their importance may diminish or increase over time. However, users are generally fully satisfied with explanations only when they effectively provide comprehensive coverage of relevant answers for all their goals \citep{sovrano2022generating}.

\subsection{Approximation with one tree} 
Decision Tree (DT) or Single Tree. It is commonly recognized that decision tree is one of the more interpretable and easily understandable models, primarily for global, but also for local, explanations. Indeed, a very widespread technique for opening the black box is the so-called “single-tree approximation” \citep{guidotti2018survey}.

\subsection{Contrastive Explanations}
Human explanations tend to be contrastive, comparing a certain factual phenomenon with a hypothetical one. In the case of decision support systems (DSS), a natural question to ask is "Why this recommendation?" This question implies a contrast, as the person asking it often has an explicit alternative in mind. In other words, the implicit question is "Why this recommendation and not that other recommendation?" The specific contrast allows the explanation to focus on the differences between the fact and the hypothesis. Humans use contrastive explanations to concisely and specifically explain events, and this advantage also applies to systems: contrastive explanations reduce the available information to a concrete difference between two outcomes. The specifics can vary depending on how the recommendation is contrasted with a different recommendation, for example, using rules or examples. In the context of a DSS recommending an insulin dose for managing type 1 diabetes, a contrastive explanation based on rules could be: "Currently, the temperature is below 10 degrees, and a lower insulin dose is recommended. If the temperature were above 30 degrees, a normal insulin dose would have been recommended." This explanation contains two rules that explicitly describe the differentiating decision boundaries between the fact and the hypothesis \citep{van2021evaluating}. In summary, facts supporting one decision are sought and counter-arguments opposing the other decision are identified \citep{padhiar2021semantic}.

\subsection{Content-Based Explanations}
Content-based explanations in recommendation systems rely on item properties and user ratings to justify recommendations. These systems use user ratings to create a classifier that represents the user's rating behavior. This classifier is then used to predict the highest ratings for recommended items \citep{tintarev2015explaining}. For example, some approaches infer a user's preferred actor based on their ratings and justify a movie recommendation based on the presence of that actor.



\subsection{Knowledge-Based Explanations}
Knowledge-based systems utilize a knowledge base and rules in an inference engine to solve problems. For example, in a knowledge-based recommendation system for cameras, properties such as memory, resolution, and price may be taken into account along with user preferences. The system can explain a camera recommendation by stating, "Less memory, lower resolution, and cheaper" \citep{tintarev2015explaining}.

\subsection{Example-Based Explanations}
Example-based explanations refer to historical situations in which the recommendation has been either true or false. For instance, "The temperature is currently 8 degrees, and a lower insulin dose is recommended. Yesterday was similar: it was 7 degrees, and the same advice turned out to be correct. Two months ago, when it was 31 degrees, a normal dose was recommended instead, which proved to be correct for that situation." Such example-based or instance-based explanations are often used among humans as they illustrate past behaviors and allow generalization to new situations \citep{van2021evaluating}.

\subsection{Contextual Explanations}
A contextual explanation provides the user with all the "external factors" that influence the decision. For example, in the given example, the season during which cauliflower is available would be considered a contextual knowledge that can be used to provide a contextual explanation, explaining why it is recommended to have potato-curry with cauliflower \citep{padhiar2021semantic}.



\subsection{Counterfactual Explanations}
Counterfactual explanations address "What if?" questions, seeking to answer whether a change would occur if the system used question parameters for a recommendation. They provide an approximation of the effects of modifying the inputs to the system. In this case, to provide an explanation, we would need to explore the effects of changing factors in the user and system profile. This can include the user's nutritional goals, preferences and dislikes, as well as any restrictive conditions such as pregnancy, allergies, and dietary requirements. For example, if a recommendation system suggests a specific dish, a counterfactual explanation could explore what would have happened if the user's preferences or constraints were different, such as in the case of pregnancy or food allergies \citep{padhiar2021semantic}.

It should be noted that contrastive explanations focus on comparing real options, whereas counterfactual explanations focus on the hypothetical consequences of changing the inputs to the system.

Most existing research has focused on exploring how users prefer a system to reason. For example, users prefer an example-based spam filter over rule-based ones \citep{pazzani2000representation}, while they prefer rule-based explanations for spam filters \citep{stumpf2009interacting}." 

\section{Evaluation of XAI Methods}

Many measures exist for computational experiments on suggested XAI methods (e.g., fidelity, sensitivity, and consistency). However, there is a lack of validated measures for user evaluations. In the literature, two main types of measures useful for user evaluations of XAI have been identified: declarative measures and behavioral measures.

\subsection{Declarative Measures}
Declarative measures are subjective and are often used in user evaluations of XAI. They provide insights into users' conscious thoughts, opinions, and perceptions. They recommend the use of declarative measures for subjective constructs (e.g., perceived understanding) but also suggest a critical perspective on whether the measures effectively address the intended constructs \citep{van2021evaluating}.

Suppose we are developing an XAI system that provides explanations for predictions made by an AI model in the medical domain. To evaluate our perception as users regarding the quality of the provided explanations, we can conduct a study where we are asked to fill out a questionnaire after interacting with the XAI system.

\subsection{Behavioral Measures}
Behavioral measures have a more observational nature and are used to measure actual behavioral effects. They recommend their use for objectively measuring constructs such as understanding and task performance. However, it is important to note that such measures often only capture one aspect of behavior \citep{van2021evaluating}.

Suppose we are developing an XAI system that generates explanations for decisions made by an AI model. To evaluate the effectiveness of this XAI system, we could conduct an experiment where we divide participants into two groups: one group uses the XAI system to obtain explanations for the model's decisions, while the other group does not have access to these explanations. We can then measure the participants' behavior, such as observing how often they request additional explanations, how many decisions they question, or how much time they spend interacting with the XAI system. These behavioral measures allow us to directly observe the effects of the XAI system on users' actual behavior when interacting with the provided explanations. They provide an objective evaluation of the impact of the XAI system on user behavior and complement the declarative measures that rely on users' subjective opinions and perceptions.

Ideally, a combination of both types of measures should be used to evaluate effects on both user perception and behavior. This way, a comprehensive perspective on a construct can be obtained. In practice, some constructs lend themselves more to declarative measures, such as user perception of confidence or understanding. Other constructs are better suited for behavioral measures, such as task performance, simulability, predictability, and persuasiveness.

Furthermore, it is recommended to measure the effects of explanations implicitly rather than explicitly. When participants are unaware of the evaluation's purpose, their responses may be more authentic. Additionally, when measuring understanding or similar constructs, explicit participant focus on the explanations can lead to biased results that do not reflect real-world application \citep{van2021evaluating}.


\newpage
\section{linked related work} 

Previous research has demonstrated that users have a growing interest in obtaining both answers and the underlying reasoning for their nutrition and food-related inquiries \citep{forbes2011content}, \citep{ueda2014recipe}, \citep{mokdara2018personalized}, \citep{ueda2011user}, \citep{el2012food}, \citep{teng2012recipe}. However, users now desire a deeper understanding of the evidence and reasoning behind these claims. In the field of food and culinary arts, efforts have been made to apply logic, reasoning, and querying techniques to capture and integrate information from diverse food-related sources \citep{haussmann2019foodkg}, \citep{haussmann2019foodkg}, \citep{batra2020recipedb}, \citep{popovski2019foodontomap}.

Existing approaches to food recommendations often rely on factors such as recipe content (e.g., ingredients) \citep{forbes2011content},\citep{el2012food}, \citep{teng2012recipe}, user behavior history (e.g., eating history) \citep{ueda2014recipe}, \citep{mokdara2018personalized}, or dietary preferences \citep{mokdara2018personalized}, \citep{ueda2011user}. However, these systems typically lack the provision of explanations for why specific food items are recommended. This limitation arises due to the utilization of black-box deep learning models, which do not offer insights into the underlying rationale behind the recommendations.

Conversely, in other domains, there are systems that employ post hoc explainable artificial intelligence (XAI) methods to provide explanations for opaque AI systems \citep{adadi2018peeking}, \citep{dovsilovic2018explainable}. However, such methods have not yet been extensively applied in the domain of food recommendation. The absence of XAI-based explanations in this domain highlights an opportunity to enhance the transparency and understanding of food recommendation systems \citep{adadi2018peeking}, \citep{dovsilovic2018explainable}. 

We were inspired by the system proposed by \citep{dragoni2020explainable}.It relies on templates, which serve as a grammar that encompasses the various elements of a persuasion message. These templates have terminal symbols organized in a hierarchical manner, with the most specific terms linked to particular persuasion strategies. A filler layer is responsible for populating the terminal symbols within the templates. Once the templates are filled, a sentence realizer generates natural language sentences that adhere to the grammatical rules of the target language. 
Our approach distinguishes itself from previous works by incorporating a higher level of explicit interpretability to food recommendations by displaying hybrid explanaition styles. This enriched approach serves as the basis for generating detailed explanations when recommending a specific food item or addressing specific questions related to a recommendation. In addition, there is a growing recognition of the importance of providing user-centered explanations that foster trust and enhance understanding of AI systems and the information they utilize for making recommendations \citep{mittelstadt2019explaining}.It also aim to address questions pragmatically, with a focus on user needs and goals \citep{sovrano2022generating}.These explanations prioritize assisting users in achieving their goals, ensuring comprehensive coverage of relevant answers for all user goals. In the pursuit of user-centered explanations, the single-tree approximation or decision trees (DT) are commonly used as interpretable models. Decision trees provide both global and local explanations and are recognized for their ease of understanding. The "single-tree approximation" technique is often employed to enhance interpretability \citep{guidotti2018survey}.Human explanations tend to be contrastive, comparing a certain factual phenomenon with a hypothetical one focusing on the differences between recommendations and alternatives. Contrastive explanations can utilize rules or examples to highlight differentiating decision boundaries \citep{van2021evaluating}. In summary, facts supporting one decision are sought and counter-arguments opposing the other decision are identified \citep{padhiar2021semantic}. 

*** Je dois justifier l'hybridation des styles, plain explanation, global et local interpretation ***


==> sections/primarelated.tex <==
This section briefly overviews the literature on recommender systems in the context of food recommender systems (Section \ref{subsec:conventional}) and evolving towards explainable and interactive recommendations (Section \ref{subsec:interactiveRecSys}).

\subsection{Conventional Food Recommendation}
\label{subsec:conventional}
One of the first concepts of a food recommender system, CHEF, dates back to 1986~\citep{Hammond1986CHEFAM}. It tests case-based planning, defining a few success/failure conditions and attempting to replace/improve food items within recipes. The cased-based planning model used in CHEF requires an extensive initial knowledge base, remarkable pre-processing, and the creation of plans and backup plans for each recipe. 
%
Freyne and Berkovsky implement the general intuition of recommender algorithms such as collaborative filtering (CF), and content-based (CB) approaches to recommend recipes~\cite{JillBerkovsky2010}. Their strategy to determine ingredient weights and use them with the CF and CB performs better when making predictions than directly using the recipes. 
%
Ge, Ricci and Massimo introduce concepts of personalization of the recommendations subordinating taste to health~\cite{Ge2015}. 
%
Chi, Chen and Tasi focus on recommending food for chronic individuals (i.e.,  kidney diseases) \cite{CHI2015208}. The authors architected a specific Ontology Web Language (OWL) ontology embedding health-relevant aspects rather than specific calculations. 
%
A more generalized healthy recommendation framework is proposed by Chen \textit{et al.}~\cite{CHEN2020102051}. It focuses on modifying unhealthy recipes from a dataset of unhealthy food. They propose a new deep learning-based method (IP-embedding) to match recipes with desired ingredients. The IP-Embedding is used to build a pseudo recipe (a set of ingredients forming the desired outcome) from the requirements, which is then matched to healthy ingredients, and finally matched with a real recipe via the MSE metric. 
%
Similarly, Teng, Lin and Adamic seeks to build a pointwise comparison metric to understand how to realize recipes from ingredients and swap them with healthier alternatives~\cite{Teng2012}. Ingredients/food substitution has also been tackled by Elsweiler, Trattner and Harvey~\cite{Elsweiler2017}. They metricize the nutritional values for fat, sodium, etc., for a predetermined healthy range. Then, images of the recipes push users to prefer healthier food rather than unhealthy options.

\subsection{Early Interactive Recommendation System} 
\label{subsec:interactiveRecSys}
Explainable AI (XAI) is pervading humans' daily lives. AI predictors and classifiers are no longer allowed to be opaque. To be trusted and make a real impact on humans, they need to be more transparent, understandable, and inspectable~\cite{anjomshoae2019explainable}. Indeed, recommender systems are expected to equip their outcomes with explanations~\cite{GunningAha2019}. Such explanations should allow for justification, control, and discovery of new aspects of the proposed outcome~\cite{AlexandraBadica2021}. 
%
Padhiar \textit{et al.} propose a food recommender system drafting explanations from knowledge-based ontology \cite{Padhiar2021}. 
%
Samih, Adadi and Berrada push the concept further, proposing a knowledge-based explainable recommender system where they generate explanations using the probabilistic soft-logic framework \cite{SamihAdadiBerrada2019}. 
%
Finally, to increase the interaction between the user and the virtual assistants, Lawo \textit{et al.} define a cluster of consumers with ethical and social priorities and include them in the recommendation process negotiation as central concerns --- recording positive feedback w.r.t. concerning the alternatives proposed \cite{Lawo2021}.

Overall, recommendation systems are not new in the nutrition domain. Pursuing healthy,  sustainable, and taste-based combinations are the most targeted goals. Recent studies tried to embed explanations in the recommendations to foster transparency --- henceforth trust and acceptability. Aligned with this trend, the following section presents an interactive communication/negotiation protocol enabling explainable mechanisms to dive into specific topics and to learn from the user's feedback promptly.


==> sections/temp.tex <==
%\subsection{Collaborative-Based Explanations}
%Collaborative-based explanations in recommendation systems utilize user ratings to find similar users (neighbors) to a given user. These neighbors are used to extrapolate a prediction about the recommended item. A famous example is Amazon's use of the explanation "Customers Who Bought This Item Also Bought..." which shows recommendations based on similar items that users are already interested in. Explanation interfaces can include graphics and text, referring to the neighbors and their ratings. These explanations are specific to the recommendation method used and assume that users provide ratings for items \citep{tintarev2015explaining}.

%\subsection{Case-Based Reasoning Explanations}
%Case-based reasoning style explanations in recommendation systems primarily focus on similar items used for making the recommendation rather than detailed item characteristics. These explanations emphasize the use of similar cases to compare and justify the recommendation. Suppose a user has recently enjoyed several Italian dishes like pizzas, pasta, and lasagna. The recommendation system, using case-based reasoning, looks for other similar users who have also had similar food preferences. By analyzing the choices of these similar users, the system identifies additional popular Italian dishes like gnocchi or risottos that might also appeal to the user in question. The explanation for this recommendation focuses on the fact that other users with similar tastes have also enjoyed these Italian dishes. By highlighting this similarity in preferences, the system aims to provide the user with a clear justification for the recommendation, allowing them to better understand why these specific dishes are being suggested \citep{tintarev2015explaining}.


 % \begin{figure*}[htp!]
 %      \centering
 %      \subfloat{
 %         \centering
 %         \includegraphics[width=\linewidth]{images/old_Interactive_VS_new_Interactive.pdf}
 %      }    
 %      \hfill
 %      \vspace{0.5pt}
 %   \begin{minipage}[b]{1\linewidth}
 %     \scriptsize
 %    \begin{tabularx}{\textwidth}{ p{.4cm} X p{1.7cm} p{.8cm}  p{0.65cm}}
 %        Id & Questions label & Metric & U & p \\\hline
 %         Q1 & The interaction interface enabled me to effectively express my feedback for the recommendations. & Sociability &   & \\
 %        Q2 & The recommender system was receptive to my feedback. &Sociability&   &  \\
 %        Q3 & The recommender system gave me enough information to decide. & Completeness &   & \\
 %        Q4 & The recommender system was easy to use. & Usability  &  & \\
 %        Q5 & I found a recipe without consuming too much time. & Usability &  & \\
 %        Q6 & The interaction with the system was smooth and effortless. & Usability &  & \\
 %        Q7 & I would like to use such a system in my daily life. & Acceptability&  & \\\hline
 %    \end{tabularx}
 %     \end{minipage}%
 %     \caption{Box plot and p-values of the first set of questions comparing new regular against new interactive}
 %     \label{fig:comparative-questions}
 % \end{figure*}



 
%\begin{figure*}[htp!]
%     \centering
%      \subfloat{
%         \centering
%         \includegraphics[width=\linewidth]{images/old_Interactive_VS_new_Interactive.pdf}
%      }    
%      \hfill
%      \vspace{0.5pt}
%   \begin{minipage}[b]{1\linewidth}
%     \scriptsize     
%    \begin{tabularx}{\textwidth}{ p{.4cm} X p{1.7cm} p{.8cm}  p{0.65cm}}
%        Id & Questions label & Metric & U & p \\\hline
%         Q1 & The interaction interface enabled me to effectively express my feedback for the recommendations. & Sociability &   1633.5 & 0.103\\
%        Q2 & The recommender system was receptive to my feedback. &Sociability&  1418.0 & 0.800 \\
%        Q3 & The recommender system gave me enough information to decide. & Completeness & 1483.0  & 0.504\\
%        Q4 & The recommender system was easy to use. & Usability  & 1377.5 & 1.0\\
%        Q5 & I found a recipe without it  consuming too much time. & Usability & 2413.5 & 8.139e-13\\
%        Q6 & The interaction with the system was smooth and effortless. & Usability & 1621.5  & 0.120 \\
%        Q7 & I would like to use such a system in my daily life. & Acceptability& 1437.0 & 0.708 \\\hline
%    \end{tabularx}
%     \end{minipage}%
%     \caption{Box plot and p-values of the first set of questions comparing old interactive  against new interactive}
%     \label{fig:old_int_vs_new_int}
% \end{figure*}



%\begin{figure}[h]
%\centering
%\includegraphics[width=1\textwidth]{images/acceptance_healthiness.png}
%  \caption{Level of healthiness of accepted food recipes per participant}
%  \label{fig:acceptance-healthiness-bar-chart}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%
\begin{table}[]
\caption{}
\label{undefined}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\hline
Interaction Type & Order             & Mean & Std  \\ \hline
Interactive      & I-\textgreater{}R & 2,27 & 0,67 \\
Interactive      & R-\textgreater{}I & 2,21 & 0,63 \\
Regular          & I-\textgreater{}R & 2,19 & 0,75 \\
Regular          & R-\textgreater{}I & 2,46 & 0,64 \\ \hline
                 &                   &      &      \\
                 &                   &      &     
\end{tabular}%
}
\end{table}

We can also observe that the learning effect is indeed minimized by the same analysis applied on the health scores of accepted food recipes rather than the questionnaire results, as illustrated by Figure \label{tab:interaction-order-healthscore}


%\begin{figure}[h]
%  \centering
% \includegraphics[width=1\textwidth]{images/explanations-questions-bar-chart.png}
%  \caption{Explanations questions bar chart}
%  \label{fig:explanations-questions-bar-chart}
%\end{figure}


    %
    %Albeit interactive session scored lower in average than the regular session, the $Q4$($p$=...), $Q5$($p$=...) and $Q6$($p$=...), shows no significant change in the usability of the system. Thus, we can draw the conclusion that the added components of an interactive session does not result in a major deterrence to participant experience. 

%Interactive->Regular stands for the participants that first started with the interactive session and then continued to regular, and the  Regular->Interactive is vice-versa.
%To investigate the results of counter sampling, and intuitively the effects of participant learning between results, we have analyzed the answers from the participants according to the order they received their sessions. Figure \ref{fig:session-order-comparative-explanations} shows the questions and the respective average answers per the order of sessions they underwent. I->R signifies that the participants first started with interactive and then regular, whereas R->I starts with regular and continues to interactive.



Most existing research in this field has focused on exploring how users prefer a system to reason. For example, users prefer an example-based spam filter over rule-based ones \citep{pazzani2000representation}, while they prefer rule-based explanations for spam filters~\cite{stumpf2009interacting}.

textbf{User-Centered Explanations}\\
This approach aims to pragmatically address a question, considering pragmatism to be synonymous with user-centeredness. It can be achieved within an explanatory process through an adequate amount of usability. In short, the definition of usability adopted in the literature is the combination of effectiveness, efficiency, and satisfaction, as per ISO 9241-210, which defines usability as ``the extent to which a system, product, or service can be used by specified users to achieve specified goals with effectiveness, efficiency, and satisfaction in a specified context of use.'' What is crucial for proper user-centeredness is to assist the user in achieving their own goals. In an explanatory process, a user's goals are identified through questions. Some questions may be explicit, while others may not be, and their importance may diminish or increase over time. However, users are generally fully satisfied with explanations only when they effectively provide comprehensive coverage of relevant answers for all their goals~\cite{sovrano2022generating}.
Some questions may be explicit and others not, some
may lose importance over time or vice versa, but normally a user is fully satisfied with explanations
only when they effectively convey full coverage of relevant answers for all of his or her goals of
understanding






 Knowledge-based systems utilize a knowledge base and rules in an inference engine to solve problems. For example, in a knowledge-based recommendation system for cameras, properties such as memory, resolution, and price may be taken into account along with user preferences. The system can explain a camera recommendation by stating, ``Less memory, lower resolution, and cheaper''~\cite{tintarev2015explaining}. One such method used in knowledge based explanations is the single tree method. Given that decision trees are inherently interpretable models, it is often instinctive to utilize them as a means to retroactively explain the a given choice. By mapping the outcomes onto decision trees, we can gain insights into why a particular result was obtained, relying on the input features as the basis for explanation \cite{guidotti2018survey}.


 
%\noindent \textbf{Approximation with one tree} 
%\noindent Decision Tree (DT) or Single Tree are commonly recognized as the most interpretable and easily understandable models, primarily for global, but also for local, explanations. Indeed, a very widespread technique for opening the black box is the so-called ``single-tree approximation''~\cite{guidotti2018survey}.


\noindent \textbf{Example-Based Explanations}
\noindent Example-based explanations refer to historical situations in which the recommendation has been either true or false. For instance, ``The temperature is currently 8 degrees, and a lower insulin dose is recommended. Yesterday was similar: it was 7 degrees, and the same advice turned out to be correct.


Two months ago, when it was 31 degrees, a normal dose was recommended instead, which proved to be correct for that situation.'' Such example-based or instance-based explanations are often used among humans as they illustrate past behaviors and allow generalization to new situations~\cite{van2021evaluating}.


\noindent \textbf{Content-Based Explanations}
\noindent Content-based explanations in recommendation systems rely on item properties and user ratings to justify recommendations. These systems use user ratings to create a classifier that represents the user's rating behavior. This classifier is then used to predict the highest ratings for recommended items~\cite{tintarev2015explaining}. For example, some approaches infer a user's preferred actor based on their ratings and justify a movie recommendation based on the presence of that actor.

\noindent A contextual explanation provides the user with all the ``external factors'' that influence the decision. In the given example, the season during which cauliflower is available would be considered a contextual knowledge that can be used to provide a contextual explanation, explaining why it is recommended to have potato-curry with cauliflower~\cite{padhiar2021semantic}.

\begin{table}[]
\caption{Examples of explanation types}
\label{tab:explanation-types-examples}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll}
\hline
Type of Explanation &
   \\ \hline
User-Centered Explanation &
  To enhance your movie-watching experience, we recommend this film based on your past preferences for action thrillers and your interest in the lead actor. \\
Contrastive Explanations &
  While customer A received a discount due to their loyalty and frequent purchases, customer B did not meet the eligibility criteria for the promotional offer \\
Content-Based Explanations &
  We suggest this song because it shares similar musical elements, such as the upbeat tempo and catchy melodies, with the songs you have enjoyed in the past \\
Knowledge-Based Explanations &
  The forecasted weather conditions are based on historical data, meteorological models, and atmospheric patterns observed in this region \\
Counterfactual Explanations &
  If you had chosen a different route, your estimated travel time would have been shorter by 15 minutes due to less traffic congestion on an alternative road \\
Example-Based Explanations &
  The spam email filter identified this message as spam because it exhibits similar characteristics, such as suspicious links and keywords, to known spam emails in our database \\
Contextual Explanations &
  Based on the current weather conditions and your location, the navigation app suggests taking a detour to avoid heavy traffic on your usual route, ensuring you reach your destination faster. \\ \hline
\end{tabular}%
}
\end{table}





%CD: do we really need the part on the evaluation of xai methods? Is it beneficial for us or just divertive? 

%Building on some of the aforementioned approaches and methods, the following section presents an interactive communication/negotiation protocol that enables explainable mechanisms to delve into specific topics and promptly learn from user feedback.

% New references/ Explain the two styles and the difference between them **********


%\section{Contrasive / counterfactual explanations}
%In recent years, there has been an increasing focus in the fields of philosophy of science on theories of contrastive explanations and counterfactual causality \citep{kment2006counterfactuals,ruben2015explaining}. These theories argue that causal explanations inherently involve the consideration of counterfactual cases, involving causes or events that did not actually occur. An example often cited is Lipton's idea that explaining why P rather than Q requires pointing out a causal difference between P and not-Q, involving a cause of P and the absence of a corresponding event in the history of not-Q \citep{lipton1990contrastive}. Some authors go as far as claiming that all questions about causality are fundamentally contrastive \citep{lewis1973counterfactuals,ruben2015explaining}.

However, contrastive theories of explanation have not been without criticism. \citep{ruben2015explaining} suggests that even if causal explanations are inherently contrastive (which he doubts), traditional theories of explanation can handle this aspect, making the "contrastive turn" interesting but ultimately unnecessary. While the usefulness of contrastive theories is still a topic of debate, the fact that contrastive explanations focus on specific events or cases and are thus simpler to generate than complete or global explanations of model functionality suggests that they should be further considered in the context of explainable artificial intelligence (xAI) \citep{lipton1990contrastive}.


Contrastive theories of explanation are of course not without criticism. Ruben (2004), for example, has suggested that, even if causal explanations are inevitably contrastive in nature (which he doubts), this characteristic can be dealt with by traditional theories of explanation, rendering the ‘contrastive turn’ interesting but
ultimately unnecessary. While the utility of contrastive theories
remains debated, the fact that contrastive explanations address a
particular event or case and are thus simpler to generate than com-
plete or global explanations of model functionality suggest they
worth further consideration in xAI (Lipton, 1990).




%Miller's review encompassed articles and empirical studies from philosophy, psychology, and cognitive science that explored how individuals define, select, evaluate, and present explanations. Three primary characteristics of explanations emerged from his analysis, highlighting their real-world usage: Human explanations are contrastive, human explanations are selective, human explanations are social.
\noindent \textbf{Contrastive Explanations}\\
\noindent Human explanations tend to be contrastive, comparing a certain factual phenomenon with a hypothetical one. In the case of decision support systems (DSS), a natural question to ask is ``Why this recommendation?''. This question implies a contrast. Indeed, the person asking for it expects an explicit alternative. In other words, the implicit question is ``Why this recommendation and not that other recommendation?''. The specific contrast allows the explanation to focus on the differences between the fact and the hypothesis. 

Humans use contrastive explanations to concisely and specifically explain events, and this advantage also applies to systems: contrastive explanations reduce the available information to a concrete difference between two outcomes. The specifics can vary depending on how the recommendation is contrasted with a different recommendation, for example, using rules or examples. In the context of a DSS recommending an insulin dose for managing type 1 diabetes, a contrastive explanation based on rules could be: ``Currently, the temperature is below 10 degrees, and a lower insulin dose is recommended. If the temperature were above 30 degrees, a normal insulin dose would have been recommended.'' This explanation contains two rules that explicitly describe the differentiating decision boundaries between the fact and the hypothesis~\cite{van2021evaluating}. In summary, facts supporting one decision are sought, and counter-arguments opposing the other decision are identified~\cite{padhiar2021semantic}.



\noindent \textbf{Counterfactual Explanations}
\noindent Counterfactual explanations address "What if?" questions, seeking to answer whether a change would occur if the system used question parameters for a recommendation. They provide an approximation of the effects of modifying the inputs to the system. In this case, to provide an explanation, we would need to explore the effects of changing factors on the user and system profile. This can include the user's nutritional goals, preferences, and dislikes, as well as any restrictive conditions such as pregnancy, allergies, and dietary requirements. For example, if a recommendation system suggests a specific dish, a counterfactual explanation could explore what would have happened if the user's preferences or constraints were different, such as in the case of pregnancy or food allergies \citep{padhiar2021semantic}. Mainly, we can consider them separately from contrastive explanations based on the fact that contrastive explanations cover real options whereas counterfactual explanations are only for hypothetical inputs.




 %\textbf{Joris's comments:}



general problem: trust and transparency. So, explainable AI, increasingly also interactive, to allow additional explanation and feedback. 

application domain: food and health; nutrition virtual coach;
as part of that wider persuasive aim, now focus on one session: recommender systems for recipes  

research question: how to design interactive explainable recommender systems for the food and health domain ?

method: \\
(1) re-designed an existing system (PRIMA), to also accommodate interactive explanations;  \\ 
(2) evaluated the system, and compared regular to interactive sessions in a within-subjects design. \\
Evaluated on objective (number of turns; reached agreement) and subjective measures (satisfaction; perceived effectiveness and usability)

results: \\
users in general are satisfied with the idea of explanations. \\
interactive sessions perform better (effectiveness) or similar (usability); this is confirmed by objective measures about number of turns and agreement 

Limitations: low number of participants, but adequate for comparisons; only initial study. \\
participants were participating in a system test; not for real food advice. so they may have been exploring. this shows e.g. in the relative length of sessions.  means it is valid as a system test comparing functionalities; not too much conclusions about persuasiveness of the food recommendations. 

take-away: promising, but the experiments  also show how difficult it is to design good explanations

Future work: multi-modal explanation (diagrams; pictures)
initiative-handling; refer to paper with Giovanni.; 
link to work on relationship building for NVC with chatbots (EREBOT) 

